Incremental Adaptive Attack Synthesis

Information leakage is a significant problem in modern software systems. Information leaks due to side channels are especially hard to detect and analyze. In this paper, we present techniques for automated synthesis of adaptive side-channel attacks that recover secret values. Our attack synthesis techniques iteratively generate inputs which, when fed to code that accesses the secret, reveal partial information about the secret based on the side-channel observations, reducing the remaining uncertainty about the secret in each attack step. Our approach is incremental, reusing results from prior iterations in each attack step to improve the efficiency of attack synthesis. We use symbolic execution to extract path constraints, automata-based model counting to estimate probabilities of execution paths, and meta-heuristics to maximize information gain based on entropy in order to minimize the number of synthesized attack steps.

==> figures/automaton_example.tex <==
%!TEX root = ../dissertation.tex
\begin{tikzpicture}[ %
      remember picture,
      auto,
      every node/.style={align=center},
      level distance=5em,
      level 1/.style={sibling distance=12em},
      level 2/.style={sibling distance=6em}
    ]

    \node (s00) [rect ,rect label={$(i,j)$}] {\input{figures/ieqjpositive}};
    \node (s04) [rect, rect label={$v$}, right = of s00] {\input{figures/charata_even}};%
  \end{tikzpicture}

==> figures/charata_even.tex <==
%!TEX root = ../../presentation.tex
\begin{tikzpicture}[->,>=stealth',shorten >=1pt, auto]
  \node[initial,initial text=,state] (A) {$0$};
  \node[state]         (B) [right of=A] {$1$};
  \node[accepting,state]         (C) [right of=B] {$2$};

  \path (A) edge [above] node {b} (B)
        (B) edge [below,bend left=30] node {$\mbox{a},\mbox{b}$} (A)
        (A) edge [above,bend left=40] node {a} (C)
        (C) edge [loop above] node {$\mbox{a},\mbox{b}$} (C);
\end{tikzpicture}


==> figures/grammar.tex <==
%!TEX root = ../../paper.tex

\begin{grammar} %
	<$\frml$> $\longrightarrow$ $\frml\AND\frml$\Alt$\frml\OR\frml$\Alt$\NOT\frml$\Alt$\frml_\Zbb$\Alt$\frml_\Sbb$\Alt$\true$\Alt$\false$ %

	<$\frml_\Zbb$> $\longrightarrow$ $\iterm=\iterm$\Alt$\iterm~\textless~\iterm$\Alt$\iterm~\textgreater~\iterm$ %
	
	<$\frml_\Sbb$> $\longrightarrow$ $\sterm=\sterm$\Alt$\sterm~\textless~\sterm$\Alt$\sterm~\textgreater~\sterm$\Alt$\match(\sterm,\rterm)$\Alt$\contains(\sterm,\sterm) %
	\alt \begins(\sterm,\sterm)$\Alt$\ends(\sterm,\sterm)$ %
	
	<$\iterm$> $\longrightarrow$ $v_i$\Alt$n$\Alt$\iterm + \iterm$\Alt$\iterm - \iterm$\Alt$\iterm \times n$ %
  \alt $\length(\sterm)$\Alt
	$\toint (\sterm)  % <------- REMOVE???
	$\Alt$\indexof(\sterm,\sterm)$\Alt$\lastindexof(\sterm,\sterm)$ %
	
	<$\sterm$> $\longrightarrow$ $v_s$\Alt$\rterm$\Alt$\sterm\cdot\sterm$\Alt$\reverse(\sterm)$\Alt$\tostring(\iterm)$\Alt$\charat(\sterm,\iterm)$\Alt$
	\alt \substring(\sterm,\iterm,\iterm)$\Alt
	$\replacefirst(\sterm,\sterm,\sterm)$\Alt$\replacelast(\sterm,\sterm,\sterm)$
	\alt $\replaceall(\sterm,\sterm,\sterm)$ %
	
	<$\rterm$> $\longrightarrow$ $\varepsilon$\Alt$s$\Alt$\rterm\cdot\rterm$\Alt$\rterm\shortmid\rterm$\Alt$\rterm^\ast$ % 
\end{grammar} %


==> figures/ieqjpositive.tex <==
%!TEX root = ../../presentation.tex
\begin{tikzpicture}[->,>=stealth',shorten >=1pt, auto]
\node[initial,initial text=,state] (s0)  {$0$};
\node[state]              (s1)           [right=2.5em of s0] {$1$};
\node[accepting,state]      (s2) [right=2.5em of s1] {$2$};
  \path (s0) edge [above] node {$(0,1)$} (s1)
        (s1) edge [bend right=50, above] node  {$(1,0)$} (s0)
        (s1) edge [loop above] node {$(1,1)$} (s1)
        (s2) edge node [above] {$(0,1)$} (s1)
        (s0) edge [bend right=30, below] node  {$(0,0)$} (s2)
        (s2) edge [loop above] node {$(0,0)$} (s2);
\end{tikzpicture}


==> tex/background.tex <==
\todo{Add content.}


==> tex/maximization.tex <==
At attack step $i$, the attacker's goal is to choose a low input $l_i$ that 
maximizes the expected information gain for that step. In the previous section 
we described how the information gain is used as an objective function to 
evaluate particular low inputs. In this section we describe different 
techniques for synthesizing attack where one simply uses satisfying model from 
ABC and other techniques use objective function maximization to find the best 
attack input 
at each step.

At a high level, our entropy maximization techniques have a common thread. In each approach, we explore a subset of the possible low inputs, and each approach is differentiated by the method used to perform this search.

One characteristic of a search is whether or not the objective function is 
evaluated for each of the low input and choose the one with the highest 
expected information gain. The techniques differ in the way the search space is 
explored. We first describe the observation query then how we use automata to 
efficiently sample from the set of feasible low inputs and after that describe 
the details of each exploration technique.

\paragraph{Observation Query}

We pick a random secret in the beginning of the attack which we want to learn 
in the end. At each step after getting a new low input we plug in both the low 
input and the secret as formula with all the path condition constraints we get 
from a program. Then, we send these updated constraints to ABC as 
satisfiability query and for one of the path condition we get it is to be 
satisfiable and we select this path as our observed path.

\paragraph{Sampling Candidate Inputs via Automata}

We send the initial path constraints to ABC and we get a satisfying model
which is the next input in the sequence. Now, we get observation of a
certain path in the program from our observation query and update the 
constraint accordingly. We again send the updated constraint to ABC and get 
satisfying model. For example, If input is BCDE and constraint of a path 
observation in the program is l[0] == h[0] \&\& l[1] != h[1], generated 
constraint for that observation for secret value is h[0] == B \&\& h[1] != C 
and for low input is l[0] == B \&\& l[1] != C where h and l are denoted as the 
secret and low input respectively. The constraint on low input is generated 
replacing the expression for h in a constraint, in this case h[0] and h[1] is 
replaced by l[0] and l[1] respectively. At the same time, we know that we 
already tried our earlier low inputs which is not the secret value. So, we add 
the constraint l != BCDE with earlier low constraint we got from the path 
observation. The updated low constraint is then sent to ABC to get model for 
the next step. This whole process is done incrementally to generate candidate 
inputs.

\paragraph{Satisfying Model}

This is the simplest form of attack synthesis where at each step we get a 
random satisfying model from ABC which we use as the next input in the 
sequence. The random satisfying model is generated based on the same process we 
discussed in the earlier section to sample candidate inputs via automata. The 
beauty of this technique is its simplicity and at the same time it does not 
consider trying different satisfying model to maximize the entropy which 
increases the number of attack steps. We will be discussing that in detail in 
the experiment section. 

\paragraph{Random Search}
We consider this technique as the base and a naive way of synthesizing an 
attack where we follow the same process of observing path and updating 
constraints but we do not consider trying low inputs as the satisfying model 
from ABC rather try from a random sample of size n. The problem with this 
approach is search space not assuring to contain at least one valid inputs for 
the updated constraints which leads to a low input with zero entropy. At that 
point, we stop the attack and we learn partial information of the secret which 
we will be explaining further in terms of remaining uncertainty in the 
experiment section. The attack also remains incomplete. We could try further 
once failing to gain information at a particular step but we did not do that as 
an approach of adaptive attack as well as we will show better techniques later 
in the paper which generates a complete adaptive attack.

\paragraph{Meta Heuristics}
We consider two different meta heuristics techniques to optimize the search 
space instead of using a random search space. These search techniques also have 
different versions in terms of searching valid and non-valid inputs against 
only valid inputs which we call unrestricted and restricted versions 
respectively. We used simulated annealing and genetic algorithm as meta 
heuristic techniques.Simulated annealing is a probabilistic technique for 
approximating global optimum of a given function. This algorithm aims to 
perturb the states according to current temperature to find better states and 
higher temperatures cause bigger perturbations. The temperature slowly cools 
down, causing the perturbations to get smaller. This temperature/cooling 
relationship lets us start with a large search space and it gets narrower as we 
spend more time searching to stay at our best solution 
\cite{simulatedannealing}.On the other hand, Genetic algorithm is an 
optimization technique where a set of candidate solutions are picked and 
evolved to generate high-quality solutions. Each candidate solution has a set 
of properties (its genes) that can be altered or mutated. Also a fitness 
function is defined to measure the success of the generated candidate 
solutions.\todo{reference for genetic algorithm}

We tried these two techniques to show that any black-box meta heuristic 
technique can be applied to the objective function we developed can lead to 
a successful attack. We show results for both these techniques in the 
experiment section.


==> tex/objective-function.tex <==
%!TEX root = ../main.tex

Here we derive an objective function to measure the amount of information
an attacker expects to gain by choosing an input value $l_{val}$ to be used in the attack
search heuristics of Section~\ref{sec:attack_synthesis_heuristics}. In the
following discussion, $H$, $L$, and $O$ are random variables representing
high-security input, low-security input, and side-channel observation
respectively. We use entropy-based metrics from the theory of quantitative
information flow~\cite{Smi09}. Given probability function
$p(h)$, 
the \emph{information entropy} of 
$H$, denoted 
$\mathcal{H}(H)$, which we interpret as the observer's \emph{uncertainty},
is 

\begin{footnotesize}
\begin{equation}
\mathcal{H}(H) = - \sum_{h \in  \mathbb{H}} p(h) \log_2 {p(h)}
\label{eq:entropy}
\end{equation}
\end{footnotesize}

\noindent Given conditional distributions $p(h | o, l)$, and $p(o|l)$ we quantify the attacker's expected \emph{updated uncertainty} about $h$, given a candidate choice of $L = l_{val}$, with the expectation taken over all possible observations, $o \in O$. We compute the  
\emph{conditional entropy of \ $H$ given $O$ with $L = l_{val}$} as

\begin{footnotesize}
\begin{equation}
\mathcal{H}(H|O, L = l_{val}) = 
-\sum_{o \in \mathbb{O}} p(o|l_{val}) \sum_{h \in \mathbb{H}} p(h | o, l_{val}) \log_2 {p( h | o, l_{val})}
\label{eq:condentropy}
\end{equation}
\end{footnotesize}



\noindent Now we can compute the expected amount of information \textit{gained} about 
$h$ by observing
$o$ after making a specific input $l_{val}$. The \emph{mutual information} between $H$ and $O$, given $L = l_{val}$ denoted $\mathcal{I}(H;O | L = l_{val})$ is the difference between the initial entropy of $H$ and the conditional entropy of $H$ given $O$ when $L = l_{val}$:

\begin{footnotesize}
\begin{equation}
\mathcal{I}(H;O | L = l_{val}) = \mathcal{H}(H) - \mathcal{H}(H | O, L = l_{val})
\label{eq:mutinfo}
\end{equation}
\end{footnotesize}

Equation~(\ref{eq:mutinfo}) serves as our objective function. Providing
input $l_{val} = l^*$ which maximizes $\mathcal{I}(H;O | L = l_{val})$
maximizes information gained about $h$. Equations~(\ref{eq:entropy})
and~(\ref{eq:condentropy}) rely on $p(h)$, $p(o|l)$, and $p(h|o,l)$, which
may change at every step of the attack. Recall that during the attack,
we maintain a constraint on the secret, $C_h$. Assuming that all secrets
that are consistent with $C_h$ are equally likely, at each step, we can
compute the required probabilities using model counting. Given a formula $F$,
performing model counting on $F$ gives the number of satisfying solutions
for $F$, which we denote $\#F$.  Thus, we observe that
$p(h) = 1 / \# C_h$ if 
$h$ satisfies $C_h$ 
and is $0$ otherwise. 
Hence, Equation~\ref{eq:entropy} reduces to 
$\mathcal{H}(H) = \log_2(\# C_h)$.

Procedure~\ref{proc:gen-constraints} gives us side-channel observations
$\mathcal{O} = \{o_1, \ldots, o_n \}$ 
and constraints over $h$ and $l$ corresponding to each $o_i$, 
$\Psi = \{ \psi_1, \ldots, \psi_n \}$. The probability that $h$ takes on a value, constrained by a particular $\psi_i$, for a given $l_{val}$ can be computed by instantiating $\psi_i$ with $l_{val}$ and then model counting. Thus, $p(h|o_i,l_{val}) = 1 / {\# (C_h \land \psi_i)[l \mapsto l_{val}]}$. 
Similarly, $p(o|l_{val}) = {\# (C_h \land \psi_i)[l \mapsto l_{val}]} / \# C_h[l \mapsto l_{val}]$.

In this paper, the \textsc{Entropy} (Equation~(\ref{eq:entropy})) and \textsc{MutualInfo} (Equation~(\ref{eq:mutinfo})) functions refer to the appropriate entropy-based computation just described, where $p(h)$, $p(o|l)$, and $p(h|o,l)$ are computed using the \textsc{ModelCount} procedure described in the next section. Using \textsc{MutualInfo}, an attacker can optimize by trying many different $l_{val}$. Observe that this process involves model counting for instantiations of string constraints for many values of $l_{val}$. In the next section we describe how to perform this model counting efficiently. 



==> tex/overview.tex <==
%!TEX root = ../main.tex
% Here we provide a high-level description of our approach. We start with an outline of how attack synthesis works and then give a brief example.



% \subsection{Measuring Uncertainty}

% One way to measure the progress of a side-channel attack is to compute
% the attacker's uncertainty about the secret at every step. Throughout
% this paper we will make use of Shannon entropy for measuring uncertainty
% and quantifying information gain~\cite{Cover2006}. We use the entropy
% formula in the coming example to demonstrate how our approach synthesizes
% a side-channel attack which incrementally decreases the uncertainty about
% the secret.  For a random variable $X$ from a sample space $\mathbb{X}$
% and probability distribution $p(X = x)$, the Shannon entropy of $X$, denoted
% $\mathcal{H}(X)$, measured in units of \emph{bits of information} is given by

% \begin{equation}
% \label{eq:entropy}
% \sum_{x \in \mathbb{X} } p(X = x) \log_2 p(X = x)
% \end{equation}


% Within the field of quantitative information flow, Shannon entropy
% is a common measure used to represent the amount of information an adversary
% has about secret information. In this paper, some variations of the
% \textsc{ChooseNextInput} functions will use the \emph{conditional Shannon
% entropy} in Section~\ref{sec:objective_function} to define an objective
% function that, when maximized, gives the input that an attacker can use
% to leak the most information about the secret.

% One particularly effective method for synthesizing attack inputs is to perform optimization over an information theoretic objective function. We use s

\subsection{PIN Checker Example}


\begin{figure}[!h]
\centering
\begin{minipage}{.72\linewidth}
\begin{lstlisting}[stepnumber=0]
public checkPIN(String h, String l){
  for (int i = 0; 4; i++)
    if (h.charAt(i) != l.charAt(i)) 
      return false;
  return true;
}
\end{lstlisting}
\end{minipage}
\caption{Pin checking example.}
\label{fig:check1}
% \vspace{-40mm}
\end{figure}



Consider a PIN-based authentication function (Figure~\ref{fig:check1}). The
PIN checking function has two inputs: 1) a secret PIN $h$, and 2)
a user input, $l$, and both $h$ and $l$ are strings of digit characters (``0''--``9'') with length $4$. Note that we have adopted the nomenclature used in
security literature. The variable $h$ denotes the {\em high-security}
value (the secret PIN) and $l$ denotes the {\em low-security} value, (the
input that the function compares with the PIN). For this example, we will
assume that the inputs are strings of length 4 consisting of characters
. The function compares the PIN and the user input
character by character and returns \texttt{false} as soon as it finds a
discrepancy. Otherwise it returns \texttt{true}.


As we now explain, \texttt{checkPIN}, one can infer information about the
secret $h$ by measuring the execution time as an observable, modeled as
the number of bytecode instructions executed. For each different length of the common prefix
of $h$ and $l$, the execution time will be different. Notice that if $h$ and $l$ have no common prefix, then \texttt{checkPIN}
will have the shortest execution time since the loop body will be executed
only once; this corresponds to executing 63 Java bytecode
instructions.  If $h$ and $l$ have a common prefix of one character, we see a longer execution time since the loop body will be executed
twice (78 instructions). In the case that $h$ and $l$ match completely, the function
has the longest running time, corresponding to 108 instructions executed
by the Java virtual machine. 





Thus, for the \texttt{checkPIN}
function there are $5$ observable values, since there will be different
execution times proportional to the length of the common prefix of $h$
and $l$.  Thus, an attacker can make inputs and use
the side-channel observations to determine how much of a prefix has matched.



We use symbolic execution to automatically map the
number of instructions executed to constraints on $h$ and
$l$~\cite{King:1976:SEP:360248.360252,Pasareanu:2013:ASE,Pasareanu:2016:MSC}.
For this example, we automatically generated path constraint that
characterize the length of the matching prefix. The path constraints and
corresponding execution costs (number of executed bytecode instructions)
is shown in Table~\ref{tab:example-pcs}. Now, by using the path constraints, along with model counting
(Section~\ref{sec:model_counting}) and one of several input search methods
(Section~\ref{sec:attack_synthesis_heuristics}), we can synthesize an
adaptive attack which determines the value of a secret PIN. The reader
can follow along in Table~\ref{tab:example-attack}.

\noindent
\begin{minipage}[!h]{0.45\textwidth}
\input{tables/example-pcs-table}
\end{minipage}
~~\begin{minipage}[!tb]{0.5\textwidth}
\input{tables/example-attack-table}
\end{minipage} \\ \\

Assuming that each PIN of the $10^4$ possible PINs are equally likely, and
applying Equation~\ref{eq:entropy}, we find that the initial uncertainty
is $13.1357$ bits of information. Suppose that the secret is ``1337''. Our
attack synthesizer generated input ``8229'' at the first step and makes
an observation with cost 63, which corresponds to $PC_1$. This in turn
indicates that ${charAt}(h,0) \not = 8$, and the uncertainty is reduced for
the next step, which is similar. At the third step we synthesized the input
``1058'', which when run gives an observation of cost 78. This indicates
that $PC_2$ is the correct path constraint to update our constraints on $h$,
which at this point would be

\vskip 1mm


\noindent $charAt(h,0) \not = 8 \land charAt(h,0) \not = 0 \land \\ charAt(h,0) = 1 \land charAt(h,1) \not = 0$ 

\vskip 1mm


We can continue synthesizing inputs and learning constraints on $h$,
which tell us more information about the prefixes of $h$, until the
uncertainty is minimized to 0 after 27 steps. At this final step,
we make an observation which corresponds to $PC_5$ indicating a full
match and the remaining uncertainty is 0. This type of attack is called
a \emph{prefix attack} or a \emph{segment attack}. These types of
attacks have been analyzed and shown to be a serious source of security
flaws~\cite{Ha09,BAP16,Xbox,CRIMEattack,Kel02,Law09.2,Nel10,Law10}. One
goal of this paper to be able to discover side-channel attacks for string
manipulating programs so that they may be mitigated before code is released.



In this paper we demonstrate and compare several techniques for synthesizing
attack inputs for string manipulating programs. As demonstrated in the
table, our search for attack inputs should drive the entropy to zero and
so we examine entropy optimization techniques. In addition, we extended
an existing  solver and model counter for string and integer constraints
called ABC~\cite{ABB15} for performing incremental string analysis, which
greatly increases the efficiency of our attack synthesis approach.



%
% \begin{figure}[htp]
% \centering
% \begin{minipage}{.72\linewidth}
% \begin{lstlisting}[stepnumber=0]
% public F2(String h, String l){
%   if(h.length != l.length)
%     return false;
%   Boolean matched = true;
%   for (int i = 0; i < h.length; i++) {
%     if (h.charAt(i) != l.charAt(i)) 
%       matched = false;
%     else 
%       matched = matched;
%   }
%   return matched;
% }
% \end{lstlisting}
% \end{minipage}
% \caption{Password checking function $F_2$.}
% \label{fig:check2}
% \end{figure}


==> tex/string-constraints.tex <==
\todo{Add content.}

